From USD Scenes to Knowledge Graphs: Zero-Shot Ontology Grounding with LLMs

Constructing knowledge graphs from 3D simulation scenes is essential for robot task reasoning, but the key bottleneck, grounding scene objects to formal ontology classes, still relies on manually curated dictionaries that are brittle and do not generalize across assets. We investigate whether large language models (LLMs) can automate this grounding step for Universal Scene Description (USD) scenes as a zero-shot, training-free alternative. On a kitchen scene (125 objects) with SOMA-HOME Ontology, LLMs achieve 90-96% exact-match accuracy with descriptive names and 49-89% with abbreviated names, substantially outperforming dictionary and embedding baselines. Under fully opaque names, context-augmented prompting recovers up to 48%. Feature ablation reveals that LLMs primarily exploit semantic cues in the scene graph (sibling names and parent paths); anonymizing these cues reduces accuracy to 0-6%, while geometry alone yields only 4-17%.

==> sections/02related.tex <==
\section{Related Work}~\label{sec:related}
Ontology-based frameworks such as KnowRob and SOMA provide the symbolic foundations for semantic reasoning in robotics, but digital twin representations such as USD remain largely geometry-centric and do not natively ground scene elements to ontology classes~\cite{beetz2018knowrob,bessler2021soma,karabulut2024ontologies}. Prior work in Multiverse addresses this by translating USD scenes into knowledge graphs using handcrafted name-to-class mappings~\cite{nguyen2024translating,nguyen2025generating}. However, these mappings are brittle, difficult to maintain, and depend heavily on controlled naming conventions. Recent LLM-based work has shown promise for ontology learning, ontology population, and 3D scene understanding, but most of these approaches rely on language or visual inputs rather than purely symbolic USD scene graphs. In contrast, our work studies whether LLMs can replace manual dictionaries for zero-shot USD-to-ontology grounding, and whether their performance reflects genuine geometric reasoning or mainly the exploitation of semantic cues already present in names and hierarchy.
